Any-Precision LLM: Low-Cost Deployment of Multiple, Different-Sized LLMs

Recently, considerable efforts have been directed towards compressing Large Language Models (LLMs), which showcase groundbreaking capabilities across diverse applications but entail significant deployment costs due to their large sizes. Meanwhile, much less attention has been given to mitigating the costs associated with deploying multiple LLMs of varying sizes despite its practical significance. Thus, this paper introduces \emph{any-precision LLM}, extending the concept of any-precision DNN to LLMs. Addressing challenges in any-precision LLM, we propose a lightweight method for any-precision quantization of LLMs, leveraging a post-training quantization framework, and develop a specialized software engine for its efficient serving. As a result, our solution significantly reduces the high costs of deploying multiple, different-sized LLMs by overlaying LLMs quantized to varying bit-widths, such as 3, 4, ..., $n$ bits, into a memory footprint comparable to a single $n$-bit LLM. All the supported LLMs with varying bit-widths demonstrate state-of-the-art model quality and inference throughput, proving itself to be a compelling option for deployment of multiple, different-sized LLMs. Our code is open-sourced and available online.

==> contents/4-algorithm-back.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/flow.pdf}
    \caption{flow}
    \label{fig:flow}
\end{figure}

\section{Any-Precision Quantization for LLM}
\label{sec:algo}
In this section, we present a methodology for a cost-effective any-precision quantization method for LLMs. We first describe how we formulate the problem of any-precision quantization (Section~\ref{sec:algo:formulation}). Then, we conduct an in-depth study on how the state-of-the-art LLM quantization methods can be utilized for any-precision quantization within the context of our defined problem (Section~\ref{sec:algo:integration}). Finally, Section~\ref{sec:algo:proposal} suggests an optimal methodology for any-precision quantization tailored for LLMs.

\subsection{Stepwise Quantization for Any-Precision Support}
\label{sec:algo:formulation}
We formulate any-precision quantization as a resolution scaling problem. Figure~\ref{fig:flow} visualizes the overall flow of our proposed method which is a two-step process. First, given a pre-trained LLM, we generate a seed model by quantizing the model into a seed bit-width ($s$-bit). $s$ can be any value between $min$ and $max$, denoting the minimum and maximum bit-width we intend to support. Any PTQ method can be employed for this step. We rule out the use of QAT method to ensure that our solution does not involve an expensive training process. Next, we upscale and/or downscale the seed model one bit at a time to generate the final set of models whose resolution ranges from $min$-bit to $max$-bit. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/upscale.pdf}
    \caption{upscale}
    \label{fig:upscale}
\end{figure}

\para{Upscaling}

Figure~\ref{fig:flow}-(b) and Figure~\ref{fig:flow}-(c) depict the process of upscaling and downscaling, respectively. Conceptually, quantization is a process of allocating values into multiple bins. Values in the same bin are rounded to the centroid of that bin. In uniform quantization methods, bins are of equal size, and centroids correspond precisely to the midpoint of the bins. In non-uniform quantization methods, the size and centroid for each bin may be arbitrarily set. Upscaling is to divide values in each bin into two groups. In uniform quantization, each bin is equally split, and the centroids are again the midpoint. In non-uniform quantization, both the split point and the centroids may be arbitrarily chosen. Downscaling is the opposite process. Two contiguous bins are merged into a single bin. Again, centroids are set to be the midpoints for uniform quantization and arbitrarily set for non-uniform quantization. The process of allocating each value into new bins during upscaling and downscaling follows the original quantization method used to produce the base resolution model, which we discuss in the following section in detail.


\subsection{Integration with SOTA Quantization Methods}
\label{sec:algo:integration}

\subsection{Analysis and Proposal}
\label{sec:algo:proposal}


%\para{Software Supports for Weight-only LLM Quantization}
%\dummypara

%\subsection{Overview}
%\label{sec:design:overview}


%\subsection{Incremental Quantization}
%\label{sec:design:quantization}

%\subsection{Bitplane-based GEMV Kernel for Non-uniform Quantization}
%\label{sec:design:kernel}

